A Hierarchical and Evolvable Benchmark for Fine-Grained Code Instruction Following with Multi-Turn Feedback

Large language models (LLMs) have advanced significantly in code generation, yet their ability to follow complex programming instructions with layered and diverse constraints remains underexplored. Existing benchmarks often prioritize functional correctness, overlooking the nuanced requirements found in real-world development. We introduce MultiCodeIF, a comprehensive benchmark designed to evaluate instruction-following in code generation across multiple dimensions: constraint type, hierarchical levels, and iterative refinement. Built upon a structured taxonomy of 9 categories and 27 constraint types, MultiCodeIF enables granular assessment of both functional and non-functional instruction adherence. Using an automated pipeline, ConstraGen, we synthesize and evolve 2,021 code tasks sourced from 14 programming languages, supporting multi-turn evaluation through feedback-driven task variants. Empirical evaluation of six state-of-the-art LLMs uncovers substantial performance disparities. The top-performing model, Claude-3-7-Sonnet, achieves 63.0% average constraint satisfaction, while smaller models like Qwen3-1.7B fall to 44.8%. Models perform well on explicit constraints, but struggle with implicit or abstract constraints. Tasks with multiple hierarchical constraints significantly reduce model success rates, from 54.5% in single-level to just 18.8% in multi-level scenarios. However, structured feedback enables progressive improvement: average constraint satisfaction rises from 63.0% to 83.4% over four iterative refinement rounds. MultiCodeIF provides a scalable, constraint-aware, and feedback-sensitive framework to benchmark LLMs under realistic code generation scenarios, bridging the gap between synthetic evaluations and real-world instruction complexity. The full benchmark dataset, evaluation pipeline, and source code are available at https://github.com/SYSUSELab/MultiCodeIF.

==> sections/comparison_datasets.tex <==
Despite recent progress in instruction datasets for code generation, existing benchmarks remain limited in three key dimensions: they are often restricted to a single programming language or popular languages (typically Python, Java, etc.), rarely support compound constraints that reflect real-world software requirements, and lack mechanisms for systematic dataset evolution. Our dataset addresses these limitations directly through a multi-language, multi-level, and compositional constraint framework, enabling more rigorous and realistic evaluation of instruction-following capabilities in LLMs.

%\input{tables/datasets_comp}

\begin{itemize}
    \item \textbf{Constraint Granularity}: Existing benchmarks often focus on functional correctness or high-level structural requirements. In contrast, our dataset introduces fine-grained constraints that mirror real development practices, including non-functional requirements, situational context, and coding conventions, enabling a more cognitively aligned evaluation of model behavior and better reflecting the full landscape of software engineering demands.
    
    \item \textbf{Evolvability and Scalability}: Our dataset is not static. It is built through an evolvable pipeline that supports (1) automatic expansion via seed code and constraint pools, and (2) systematic construction of multi-level, compound constraint tasks by building upon existing instructions. This enables efficient generation of new, progressively complex instruction-following tasks over time.
    
    \item \textbf{Multi-Level Constraint Modeling}: Our benchmark introduces a progressive constraint composition mechanism. For selected constraint categories, we define multi-level ladders where each level incrementally tightens the instruction space. This design enables evaluation of LLM performance under increasingly complex constraint conditions and obtain the limit of the model instruction following ability.

    \item \textbf{Multi-Language Support}: Our dataset includes code generation tasks across 12 programming languages, including popular Python, Java, C++, JavaScript, as well as less popular Rust, Haskell, etc. This can facilitate cross-lingual evaluation and reflecting the diversity of real-world software ecosystems.
    
    \item \textbf{Non-Leakage Guarantee}: Given that many existing datasets have become widely used in training or fine-tuning large models, leakage is a growing concern in model evaluation. Our dataset is newly constructed and has not been publicly exposed, ensuring a clean evaluation environment and higher reliability in performance attribution.
\end{itemize}

